CountGD++: Generalized Prompting for Open-World Counting

The flexibility and accuracy of methods for automatically counting objects in images and videos are limited by the way the object can be specified. While existing methods allow users to describe the target object with text and visual examples, the visual examples must be manually annotated inside the image, and there is no way to specify what not to count. To address these gaps, we introduce novel capabilities that expand how the target object can be specified. Specifically, we extend the prompt to enable what not to count to be described with text and/or visual examples, introduce the concept of `pseudo-exemplars' that automate the annotation of visual examples at inference, and extend counting models to accept visual examples from both natural and synthetic external images. We also use our new counting model, CountGD++, as a vision expert agent for an LLM. Together, these contributions expand the prompt flexibility of multi-modal open-world counting and lead to significant improvements in accuracy, efficiency, and generalization across multiple datasets. Code is available at https://github.com/niki-amini-naieni/CountGDPlusPlus.

==> figures/automatic-generation.tex <==
\begin{figure}[h!]
  \centering
  \includegraphics[width=\linewidth]{figures/automatic_generation.pdf}
  \caption{Automatic Generation}
  \label{fig:automatic_generation}
\end{figure}

==> figures/external-exemplar-encoding.tex <==
\begin{figure}[h!]
  \centering
  \includegraphics[width=\linewidth]{figures/external_exemplar_encoding.pdf}
  \caption{External Exemplar Encoding}
  \label{fig:external_exemplar_encoding}
\end{figure}

==> figures/external-exemplars.tex <==
\begin{figure}[h!]
  \centering
  \includegraphics[width=\linewidth]{figures/external_exemplars.pdf}
  \caption{External Exemplars}
  \label{fig:external_exemplars}
\end{figure}

==> figures/inference.tex <==
\begin{figure}[h!]
  \centering
  \includegraphics[width=\linewidth]{figures/inference_fig.pdf}
  \caption{Inference filtering procedure. At inference, object queries with higher maximum similarity to the negative class (strawberry) features than to the positive class (blueberry) features are removed.}
  \label{fig:inference}
\end{figure}

==> figures/training.tex <==
\begin{figure}[h!]
  \centering
  \includegraphics[width=\linewidth]{figures/training-figure.pdf}
  \caption{Contrastive training strategy. Object queries corresponding to particular (positive) visual exemplar and text prompts are pushed closer to their features and away from unrelated (negative) visual exemplar and text prompts.}
  \label{fig:training}
\end{figure}
